Point-of-Interest Type Inference from Social Media Text

Physical places help shape how we perceive the experiences we have there. For the first time, we study the relationship between social media text and the type of the place from where it was posted, whether a park, restaurant, or someplace else. To facilitate this, we introduce a novel data set of $\sim$200,000 English tweets published from 2,761 different points-of-interest in the U.S., enriched with place type information. We train classifiers to predict the type of the location a tweet was sent from that reach a macro F1 of 43.67 across eight classes and uncover the linguistic markers associated with each type of place. The ability to predict semantic place information from a tweet has applications in recommendation systems, personalization services and cultural geography.

==> otherTablesAndFIgures.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% MAP %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[h]
\centering
\includegraphics[width=0.8\textwidth]{images/map.png}
\caption{Location of tweets by category in the training set}
\label{fig:map}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% END MAP %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%
%LIWC Features TABLE
% \begin{table}[]
% \small
% \centering
% \begin{tabular}{|l|l|l|l|}
% \hline
% \rowcolor[HTML]{9B9B9B} 
% \multicolumn{2}{|c|}{\cellcolor[HTML]{9B9B9B}\textbf{Arts \& Entertainment}} & \multicolumn{2}{c|}{\cellcolor[HTML]{9B9B9B}\textbf{College \& University}}                                                  \\ \hline
% \rowcolor[HTML]{C0C0C0} 
% \textbf{feature}                         & \textbf{r}                        & \textbf{feature}                                                 & \textbf{r}                                                \\ \hline
% SAD                                      & 0.048                             & NONFLU                                                           & 0.095                                                     \\ \hline
% FRIEND                                   & 0.045                             & HEALTH                                                           & 0.037                                                     \\ \hline
% COGPROC                                  & 0.039                             & PREP                                                             & 0.035                                                     \\ \hline
% ACHIEVE                                  & 0.033                             & REWARD                                                           & 0.028                                                     \\ \hline
% AFFILIATION                              & 0.026                             & CAUSE                                                            & 0.024                                                     \\ \hline
% IPRON                                    & 0.025                             & SWEAR                                                            & 0.022                                                     \\ \hline
% ADJ                                      & 0.025                             & FAMILY                                                           & 0.016                                                     \\ \hline
% CAUSE                                    & 0.024                             & POSEMO                                                           & 0.015                                                     \\ \hline
% FEEL                                     & 0.023                             & FOCUSPAST                                                        & 0.015                                                     \\ \hline
% POSEMO                                   & 0.022                             & SAD                                                              & 0.014                                                     \\ \hline
% FOCUSPRESENT                             & 0.021                             & QUANT                                                            & 0.014                                                     \\ \hline
% \rowcolor[HTML]{9B9B9B} 
% \multicolumn{2}{|c|}{\cellcolor[HTML]{9B9B9B}\textbf{Food}}                  & \multicolumn{2}{c|}{\cellcolor[HTML]{9B9B9B}\textbf{Great Outdoors}}                                                         \\ \hline
% \rowcolor[HTML]{C0C0C0} 
% \textbf{feature}                         & \textbf{r}                        & \textbf{feature}                                                 & \textbf{r}                                                \\ \hline
% FEMALE                                   & 0.222                             & NONFLU                                                           & 0.046                                                     \\ \hline
% INTERROG                                 & 0.166                             & ANX                                                              & 0.040                                                     \\ \hline
% NETSPEAK                                 & 0.016                             & INGEST                                                           & 0.036                                                     \\ \hline
% RISK                                     & 0.011                             & CONJ                                                             & 0.033                                                     \\ \hline
% SAD                                      & 0.011                             & DRIVES                                                           & 0.027                                                     \\ \hline
% CERTAIN                                  & 0.011                             & WE                                                               & 0.026                                                     \\ \hline
% SEE                                      & 0.010                             & NETSPEAK                                                         & 0.025                                                     \\ \hline
% ACHIEVE                                  & 0.010                             & ARTICLE                                                          & 0.022                                                     \\ \hline
% CONJ                                     & 0.010                             & ASSENT                                                           & 0.021                                                     \\ \hline
% MALE                                     & 0.007                             & DEATH                                                            & 0.021                                                     \\ \hline
% REWARD                                   & 0.007                             & FOCUSPAST                                                        & 0.020                                                     \\ \hline
% \rowcolor[HTML]{9B9B9B} 
% \multicolumn{2}{|c|}{\cellcolor[HTML]{9B9B9B}\textbf{Nightlife Spot}}        & \multicolumn{2}{c|}{\cellcolor[HTML]{9B9B9B}\textbf{\begin{tabular}[c]{@{}c@{}}Professional \&\\ Other Places\end{tabular}}} \\ \hline
% \rowcolor[HTML]{C0C0C0} 
% \textbf{feature}                         & \textbf{r}                        & \textbf{feature}                                                 & \textbf{r}                                                \\ \hline
% SEXUAL                                   & 0.061                             & I                                                                & 0.122                                                     \\ \hline
% ASSENT                                   & 0.045                             & DRIVES                                                           & 0.109                                                     \\ \hline
% HEAR                                     & 0.039                             & NEGEMO                                                           & 0.098                                                     \\ \hline
% CAUSE                                    & 0.023                             & INSIGHT                                                          & 0.070                                                     \\ \hline
% SAD                                      & 0.016                             & DISCREP                                                          & 0.062                                                     \\ \hline
% RISK                                     & 0.015                             & AFFILIATION                                                      & 0.053                                                     \\ \hline
% FOCUSPAST                                & 0.015                             & FEMALE                                                           & 0.051                                                     \\ \hline
% HEALTH                                   & 0.014                             & FOCUSPAST                                                        & 0.045                                                     \\ \hline
% FUNCTION                                 & 0.014                             & PREP                                                             & 0.039                                                     \\ \hline
% CERTAIN                                  & 0.011                             & FEEL                                                             & 0.036                                                     \\ \hline
% HOME                                     & 0.011                             & MONEY                                                            & 0.036                                                     \\ \hline
% \rowcolor[HTML]{9B9B9B} 
% \multicolumn{2}{|c|}{\cellcolor[HTML]{9B9B9B}\textbf{Shop \& Service}}       & \multicolumn{2}{c|}{\cellcolor[HTML]{9B9B9B}\textbf{Travel \& Transport}}                                                    \\ \hline
% \rowcolor[HTML]{C0C0C0} 
% \textbf{feature}                         & \textbf{r}                        & \textbf{feature}                                                 & \textbf{r}                                                \\ \hline
% INFORMAL                                 & 0.082                             & ANGER                                                            & 0.026                                                     \\ \hline
% SEE                                      & 0.029                             & THEY                                                             & 0.026                                                     \\ \hline
% ADJ                                      & 0.024                             & PPRON                                                            & 0.025                                                     \\ \hline
% TIME                                     & 0.020                             & MALE                                                             & 0.020                                                     \\ \hline
% FOCUSFUTURE                              & 0.018                             & NETSPEAK                                                         & 0.018                                                     \\ \hline
% DISCREP                                  & 0.016                             & POWER                                                            & 0.016                                                     \\ \hline
% HEALTH                                   & 0.016                             & FUNCTION                                                         & 0.013                                                     \\ \hline
% FOCUSPRESENT                             & 0.013                             & SEE                                                              & 0.012                                                     \\ \hline
% I                                        & 0.013                             & NEGATE                                                           & 0.011                                                     \\ \hline
% RELATIV                                  & 0.013                             & ARTICLE                                                          & 0.008                                                     \\ \hline
% SAD                                      & 0.012                             & WORK                                                             & 0.007                                                     \\ \hline
% \end{tabular}
% \caption{LIWC Features associated with each category place, sorted by Pearson correlation (r) computed between the normalized frequency of each feature and the category label across all tweets.}
% \label{tab:liwc}
% \end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%Emotion NRC%%%%%%%%%
\begin{figure}[h]
\centering
\includegraphics[width=0.9\textwidth]{images/nrc_chart.png}
\caption{NRC emotions by category}
\label{fig:map}
\end{figure}

% \begin{figure}[!h]
%      \centering
%      \includegraphics[width=0.9\columnwidth]{images/topwords_nrc.png}
%      \caption{Features with the highest values by place category for the test chi-squared statistic from words that appear in at least 5 different places and words in the NRC lexicon}
% \label{fig:topwords}
% \end{figure}

==> table-features.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%LA CHI2 +5 %%%%%%%%%
\begin{table}[t!]
\scriptsize
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
\rowcolor[HTML]{9B9B9B} 
\multicolumn{2}{|c|}{\cellcolor[HTML]{9B9B9B}\textbf{Arts \& Entertainment}} & \multicolumn{2}{c|}{\cellcolor[HTML]{9B9B9B}\textbf{Nightlife Spot}} & \multicolumn{2}{c|}{\cellcolor[HTML]{9B9B9B}\textbf{College \& University}} & \multicolumn{2}{c|}{\cellcolor[HTML]{9B9B9B}\textbf{Professional \& Other Places}} \\ \hline
\rowcolor[HTML]{C0C0C0} 
feature                     & \textbf{$\chi^2$}                     & feature                 & \textbf{$\chi^2$}                 & feature                     & \textbf{$\chi^2$}                    & feature                        & \textbf{$\chi^2$}                        \\ \hline
concert                              & 167.20                                & \#craftbeer                      & 425.97                            & campus                               & 298.74                               & school                                  & 87.46                                    \\ \hline
\rowcolor[HTML]{EFEFEF} 
museum                               & 152.14                                & '2beersE'                        & 311.68                            & college                              & 266.63                               & students                                & 79.93                                    \\ \hline
show                                 & 134.39                                & beer                             & 203.57                            & university                           & 155.65                               & grade                                   & 66.05                                    \\ \hline
\rowcolor[HTML]{EFEFEF} 
night                                & 104.48                                & bar                              & 93.90                             & class                                & 112.23                               & vote                                    & 65.80                                    \\ \hline
tonight                              & 80.76                                 & 'beerE'                          & 67.00                             & semester                             & 103.19                               & our                                     & 63.12                                    \\ \hline
\rowcolor[HTML]{EFEFEF} 
game                                 & 73.56                                 & 'wineE'                          & 56.94                             & football                             & 59.24                                & jv                                      & 60.64                                    \\ \hline
art                                  & 69.77                                 & dj                               & 56.56                             & student                              & 57.86                                & church                                  & 52.97                                    \\ \hline
\rowcolor[HTML]{EFEFEF} 
$<$mention$>$                        & 66.14                                 & tonight                          & 53.39                             & classes                              & 57.37                                & hs                                      & 50.63                                    \\ \hline
zoo                                  & 66.09                                 & ale                              & 52.62                             & students                             & 56.98                                & senior                                  & 50.05                                    \\ \hline
\rowcolor[HTML]{EFEFEF} 
baseball                             & 62.90                                 & party                            & 51.14                             & camp                                 & 44.19                                & ss                                      & 44.46                                    \\ \hline
\rowcolor[HTML]{9B9B9B} 
\multicolumn{2}{|c|}{\cellcolor[HTML]{9B9B9B}\textbf{Food}}                           & \multicolumn{2}{c|}{\cellcolor[HTML]{9B9B9B}\textbf{Shop \& Service}}         & \multicolumn{2}{c|}{\cellcolor[HTML]{9B9B9B}\textbf{Great Outdoors}}                 & \multicolumn{2}{c|}{\cellcolor[HTML]{9B9B9B}\textbf{Travel \& Transport}}                   \\ \hline
\rowcolor[HTML]{C0C0C0} 
feature                              & $\chi^2$                              & feature                          & $\chi^2$                          & feature                              & $\chi^2$                             & feature                                 & $\chi^2$                                 \\ \hline
chicken                              & 375.52                                & mall                             & 462.03                            & beach                                & 591.81                               & airport                                 & 394.20                                   \\ \hline
\rowcolor[HTML]{EFEFEF} 
\#nola                                & 340.64                                & store                            & 403.00                            & 'waveE'                              & 239.00                               & 'planeE'                                & 343.30                                   \\ \hline
lunch                                & 255.98                                & shopping                         & 359.00                            & hike                                 & 227.91                               & flight                                  & 292.94                                   \\ \hline
\rowcolor[HTML]{EFEFEF} 
fried                                & 216.49                                & shop                             & 132.39                            & lake                                 & 193.58                               & hotel                                   & 168.38                                   \\ \hline
dinner                               & 203.65                                & 'flowerE'                        & 126.07                            & park                                 & 165.92                               & conference                              & 141.74                                   \\ \hline
\rowcolor[HTML]{EFEFEF} 
'burgerE'                            & 195.41                                & 'megaphoneE'                     & 95.32                             & island                               & 151.45                               & landed                                  & 118.05                                   \\ \hline
pizza                                & 190.83                                & apple                            & 88.74                             & sunset                               & 142.44                               & plane                                   & 88.42                                    \\ \hline
\rowcolor[HTML]{EFEFEF} 
shrimp                               & 188.77                                & market                           & 76.60                             & hiking                               & 137.74                               & bound                                   & 78.43                                    \\ \hline
'pizza'                              & 179.39                                & auto                             & 73.52                             & beautiful                            & 109.45                               & heading                                 & 62.09                                    \\ \hline
\rowcolor[HTML]{EFEFEF} 
'happyE'                             & 151.00                                & stock                            & 72.31                             & bridge                               & 108.56                               & headed                                  & 57.12                                    \\ \hline
\end{tabular}
\caption{Unigrams associated with each category, sorted by $\chi^2$ value computed between the normalized frequency of each feature and the category label across all tweets in the training set ($p<0.001$)}
\label{tab:linguisticanalysis}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
